On Mitigating Code LLM Hallucinations with API Documentation

In this study, we address the issue of API hallucinations in various software engineering contexts. We introduce CloudAPIBench, a new benchmark designed to measure API hallucination occurrences. CloudAPIBench also provides annotations for frequencies of API occurrences in the public domain, allowing us to study API hallucinations at various frequency levels. Our findings reveal that Code LLMs struggle with low frequency APIs: for e.g., GPT-4o achieves only 38.58% valid low frequency API invocations. We demonstrate that Documentation Augmented Generation (DAG) significantly improves performance for low frequency APIs (increase to 47.94% with DAG) but negatively impacts high frequency APIs when using sub-optimal retrievers (a 39.02% absolute drop). To mitigate this, we propose to intelligently trigger DAG where we check against an API index or leverage Code LLMs' confidence scores to retrieve only when needed. We demonstrate that our proposed methods enhance the balance between low and high frequency API performance, resulting in more reliable API invocations (8.20% absolute improvement on CloudAPIBench for GPT-4o).

==> sections/acknowledgements.tex <==
\section*{Acknowledgements}

We will identify acknowledgements in a non-anonymous version of this paper.


==> sections/intro_back.tex <==
% \interfootnotelinepenalty=10000

\section{Introduction}


\begin{figure*}
    \centering
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{figures/introduction/api-hallucination.pdf}
        \caption{\textbf{API Hallucinations. }A task from \bench for the AWS API \texttt{bedrock.create\_model\_customization\_job} (yellow) and the output (remaining text) from StarCoder2-7B are shown. The model generates a non-existent API (red) indicating an API hallucination.}
        \label{fig:introduction-api-hallucination}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.5\textwidth}
        \includegraphics[width=\textwidth]{figures/introduction/perplexity.pdf}
        \caption{\textbf{Perplexity over API Tokens} (lower is better)\textbf{.} Code LLMs can easily invoke high frequency APIs while they struggle with low frequency APIs. While DAG (50\% retrieval precision) improves performance on low frequency APIs, it comes at the cost of high frequency API performance due to irrelevant augmentations. The methods and analyses discussed in this paper address this limitation of DAG. Results from StarCoder2-7B.}
        \label{fig:introduction-perplexity-analysis}
    \end{subfigure}
    \caption{\textbf{Motivation.} Code LLMs suffer from API hallucinations for several real-world APIs. We develop \bench to quantify API hallucinations, and present various strategies to optimize performance on \bench.}
\end{figure*}



% \nihal{
% Want to convey in the introduction:

% 1. API hallucinations are a problem. This paper presents an evaluation benchmark to measure this in context of some of the most popular API providers. We show that SoTA models suffer from this.

% 2. Humans use documentation to adapt to evolving APIs. We investgate how LLMs can use documentation.

% 3. Using documentation is not free from challenges: RAG can be ineffective with imprecise retrievers. We show how unconditional RAG can improve performance on certain APIs while degrading performance on others. We also discuss and conduct experiments that can help recover from the deficiencies of imprecise documentation retrievals.
% }


Large Language Models for code generation (Code LLMs) are being actively used by real-world programmers~\cite{peng2023impact,chen2021evaluating,dakhel2023github}. 
To develop new software, programmers often use third-party Application Programming Interfaces (APIs) as building blocks. 
A major challenge in API driven development is that APIs evolve rapidly, often at an enormous pace~\cite{mcdonnell2013empirical}---with frequent introductions, modifications, and deprecation. In this paper, we investigate and improve the ability of Code LLMs to adapt to such changes in software.

Code LLMs that are not sufficiently trained on code for new, updated or less popular APIs (\ie, \textit{low frequency} APIs) may generate incorrect code for these (see Figure~\ref{fig:introduction-api-hallucination}) because these are not adequately represented in the pre-training datasets.
We refer to such invalid API invocations as \textit{hallucinations}, signifying the Code LLMs' limitations in adapting to API evolution. In order to quantify the occurrence of API hallucinations, we introduce a new benchmark, \textbf{\bench}, focusing on APIs offered by various cloud service providers such as Amazon Web Services (AWS) and Microsoft Azure.

Amidst this evolving setting, human developers rely heavily on API documentation to remain  up to date. Likewise, Code LLMs should also refer to API documentations, especially for new APIs. Towards this, we adapt Retrieval Augmented Generation (RAG) to incorporate documentation, \ie, \textbf{Documentation Augmented Generation (DAG)}, which has shown early promise to address API hallucinations~\citep{zhou2023docprompting, patil2023gorilla}.

However, DAG may not be necessary when the intended APIs are \textit{not} updated or the Code LLM is sufficiently familiar with the API due to adequate training (\ie, \textit{high frequency} APIs). In fact, in some cases, DAG can hurt the underlying Code LLM's performance when retrievals are inaccurate because LLMs are known to be sensitive to irrelevant augmentations~\citep{irrelevant-augmentations}. As such, in this work, we not only identify where DAG can fail but also show how simple yet effective techniques can help mitigate such issues.

We illustrate how frequency of occurrence of an API in the pre-training dataset can influence Code LLMs in Figure~\ref{fig:introduction-perplexity-analysis}. We show the perplexity of StarCoder2-7B~\citep{lozhkov2024starcoder} ("Base Model") over the API name tokens for two frequency groups of APIs:  \textit{low} ($\leq 10$ occurrences in pre-training dataset) and \textit{high} ($\geq 1000$) (see Appendix~\ref{sec:appendix-api-hallucinations} for more details). 
The base model performs notably better in invoking high-frequency APIs compared to low-frequency ones. While DAG improves performance for low-frequency APIs, there's a discernible compromise in performance on high-frequency ones, indicating a trade-off. 
This trade-off arises because imperfect retrievers sometimes introduce irrelevant augmentations, diverting the attention of the Code LLM from its intrinsic knowledge. 
Hence, we explore methods such as utilizing model confidence scores~\citep{jiang2023active, varshney2023stitch} or checking the model's generation against an index before retrieval to mitigate DAG's limitations.

% For such evaluations, we present \bench, a benchmark designed to evaluate the accuracy of real-world API calls with respect to their occurrence frequency in the training dataset. 
% \bench enables us to conduct detailed analyses to explore the relationship between the frequency of an API's appearance in training data and its documentation's importance to the Code LLM. 

% \bench leverages the APIs provided by Amazon Web Services (AWS) in Python through \texttt{boto3}, one of the most downloaded Python packages~\cite{TopPyPI2024}. It contains 200+ diverse services spanning areas like cloud computing and data storage. We use the StarCoderBase~\citep{li2023starcoder} models which are pre-trained on 80+ programming languages from the Stack dataset~\citep{TheStack}. Since both the model and dataset are publicly available, it allows us to easily conduct our analyses concerning the frequencies of APIs in the pre-training dataset.

We summarize our main contributions and the paper organization below:
\begin{itemize}[leftmargin=*]
    \itemsep0em
    \item We highlight the problem of hallucinations for real-world APIs, and present \bench, a benchmark to measure API hallucinations for a diverse range of APIs offered by cloud service providers such as AWS and Azure (\textbf{Section~\ref{sec:api-hallucinations-cloudapibench}}).
    \item We investigate DAG to optimize performance on \bench by thoroughly studying 
    how various DAG components affect model performance (\textbf{Section~\ref{sec:documentation-augmented-generation}}).
    \item We characterize the conditions under which DAG can hurt model performance and explore various methods that can help improve Code LLMs' abilities to utilize documentation (\textbf{Section~\ref{sec:improving-dag}}).
\end{itemize}

Finally, we present the scope for future research in \textbf{Section~\ref{sec:conclusion}}, and discuss the limitations of our work in \textbf{Section~\ref{sec:limitations}}. 

We believe this is the first study to measure and characterize real-world API hallucinations for a range of Code LLMs, and explore various strategies to mitigate this issue using documentation.

